Compression and In-Situ Query Processing for Fine-Grained Array Lineage

Tracking data lineage is important for data integrity, reproducibility, and debugging data science workflows. However, fine-grained lineage (i.e., at a cell level) is challenging to store, even for the smallest datasets. This paper introduces DSLog, a storage system that efficiently stores, indexes, and queries array data lineage, agnostic to capture methodology. A main contribution is our new compression algorithm, named ProvRC, that compresses captured lineage relationships. Using ProvRC for lineage compression result in a significant storage reduction over functions with simple spatial regularity, beating alternative columnar-store baselines by up to 2000x}. We also show that ProvRC facilitates in-situ query processing that allows forward and backward lineage queries without decompression - in the optimal case, surpassing baselines by 20x in query latency on random numpy pipelines.

==> ack.tex <==
\section{Acknowledgment}
TODO

==> conclusion.tex <==
\section{Conclusion}

In this paper, we presented a lineage index, \sys. \sys introduces a novel lineage compression technique, \FMain, an in-situ query algorithm over the compressed provenance, and a provenance capture reuse algorithm. These optimizations introduced in \sys are an essential part of a complete system for leveraging fine-grained provenance for reproducibility and reliability in array pipelines.

==> coverletter.tex <==
\section*{Author Response}
We thank the reviewers for their helpful feedback and have addressed all of the requirements for revision. To summarize the changes:
\begin{itemize}
    \item We have significantly expanded the experiments to include one new baseline, larger scales of data, and diversity of workloads.
    \item We have included a proof of correctness in the paper to prove that the core compression algorithm is lossless.
    \item We have revised the notation and terminology to make the paper more clear.
\end{itemize}
Below, we address individual points listed by the reviewers.

\section*{Reviewer 1}

\subsection*{01. Re. Source code of DSLog should be made available.}
Done. The entire codebase used for this paper can be found at: \url{https://github.com/j2zhao/tracked_numpy}. This includes code for DSLog algorithms, experiments, baselines, and prototype lineage capture systems (including a tracked modified version of NumPy). We are working on cleaning up this codebase to package the DSLog source code separately.

\section*{Reviewer 2}
\subsection*{01. Re. Materializing the linage with tensors or numpy array in memory and perform tensor operations.}
Done (refer to Table VIII and Figure 9). While this is a very sensible approach, considering that the data are originally numpy arrays, we find that array and tensor formats do not exploit the sparsity of certain lineage operations. Even with dense input vectors, the lineage relationships between indices can be sparse. Furthermore, queries across a series of operations (where input indices have to be aligned to output indices, i.e., a join operation) are slow since we lose standard join optimizations present in most databases. In short, even though the original data is structured in multidimensional arrays, storing the lineage in a relational format is more natural to take advantage of database optimizations.

\subsection*{01. Re. Larger scale of datasets or demonstrating tensor operations cannot outperform the ProvRC in the paper. }
Done (refer to Table VII and Table VIII). We include the lineage for two SQL queries over the full IMDB dataset (rather than a subset as in previous experiments). The join query has a Raw (uncompressed) lineage of $>$2GB. We further include a linear algebra query matrix multiplication where the Raw (uncompressed) lineage is over 40GB.


\subsection*{03. Re. Experiments are still quite limited in showing the benefit of the proposed solution in the general machine learning environment. }
Done (See Section VII.C). We added a workflow over a block of the ResNet network. This Resnet workflow contains seven steps of a ResNet block during machine learning inference. This includes two convolution layers, two ReLu operations, two normalization operations, and one residual operation. These operations were greatly compressed with ProvRC, resulting in fast query times in our experiment.

\section*{Reviewer 3}
\subsection*{O1. Re. Missing from the paper are discussions of correctness of the approaches.}
Done (Section IV.B). Intuitively, the compression algorithm represents a table of integers as a union of Cartesian products (i.e., decomposes the table into a collection of all-to-all relationships). This is completely lossless under set semantics. The correctness of the query algorithm in Section V follows from the lossless aspect of the compression algorithm.

\subsection*{O2. Re. The paper could spend more time describing the notations used (section IV) prior to the definitions, etc}

Done (See preface of Section IV). We also cleaned up the notation concerning attributes, sets, and ranges.

\subsection*{O3. Re. Similarly, explaining in more detail range join would be good (as opposed to just giving a reference).}

Done (See Section V.B).

\subsection*{D1. Re. There is a typo in the running example, top of second column of page 3, in which the index should be (1,1) not (1,2).}

Done.

\subsection*{D2. Re. I think it would help the exposition if a slightly more complicated running example was used.}

For the current version of the paper, we decided to keep the current running example but expand the discussion around it e.g., Section V.B. If the reviewer insists, this could be easily updated for the camera-ready if the reviewer could give further feedback on what kind of example they would like to see.

\subsection*{D3. Re. In terms of the evaluation, it seems like the numpy operations used are favorable for the evaluation. Was any work done to see how frequently these specific operations are used in practice? If not, some discussion on this would be good..}

Done. We included a brief discussion on the selected numpy operations for storage experiments (VII.C). For the rest of the experiments, we include coverage over the entire numpy library as long as the operations met the needed criteria (VII.D and VII.E).


